High-voltage solution in radial power networks:Existence, properties and equivalent algorithms

The AC power flow equations describe the steady-state behavior of the power grid. While many algorithms have been developed to compute solutions to the power flow equations, few theoretical results are available characterizing when such solutions exist, or when these algorithms can be guaranteed to converge. In this paper, we derive necessary and sufficient conditions for the existence and uniqueness of a power flow solution in balanced radial distribution networks with homogeneous (uniform $R/X$ ratio) distribution lines. We study three distinct solution methods: fixed point iterations}, convex relaxations, and energy functions we show that the three algorithms successfully find a solution if and only if a solution exists. Moreover, all three algorithms always find the unique high-voltage solution to the power flow equations, the existence of which we formally establish.}%, which can be formally defined as the high-voltage solution -- any other solution of the power flow equations has smaller or equal voltage magnitudes at every bus. At this solution, we prove that (i) voltage magnitudes are increasing functions of the reactive power injections, (ii) the solution is a continuous function of the injections, and (iii) the solution is the last one to vanish as the system is loaded past the feasibility boundary.

==> Applications.tex <==
\section{Applications}\label{sec:Applications}


==> BackgroundFormulation.tex <==
\section{Background and Mathematical formulation}\label{sec:MathFormulation}


We study systems of quadratic equations that are parameterized affinely in a parameter $u$:
\begin{align}
f\br{x,u}=\underbrace{Q\qud{x}{x}{u}}_{\text{Quadratic terms}}+\underbrace{L\br{x,u}}_{\text{Linear terms}}+\underbrace{c\br{u}}_{\text{Constant terms}}=0 \label{eq:Quad}
\end{align}
where $Q: \R^n \times \R^n \times \R^k \mapsto \R^n$ is a tri-linear function (linear in each of its inputs for fixed values of the other inputs) with $Q\qud{0}{0}{u}=0 \quad \forall u \in \R^k$ and represents the quadratic terms in $x$, $L:\R^n \times \R^k \mapsto \R^n$ is a bi-linear function with $L(0,u)=0 \quad \forall u\in\R^k$ that  represents the linear terms in $x$, and $c: \R^n\mapsto \R^n$ is a linear function represents the constant terms in $x$.

Note that since quadratic forms can always be represented using symmetric matrices, we can assume that $Q$ is symmetric in its first two arguments:
\[Q\qud{x}{y}{u}=Q\qud{y}{x}{u} \quad \forall x,y \in \R^n,u \in \R^k\]
We view \eqref{eq:Quad} as a system of quadratic equations in $x$ parameterized by $u$ and seek to define conditions on $u$ that guarantee the existence of a solution for $x$ within $\Xcal$, a compact convex set. We use $\mathrm{Int}(\Xcal)$ to denote the interior of the set $\Xcal$.

%\begin{definition}[Jacobian]
%The Jacobian of the function $f$ is a function $J:\R^n \times \R^k \mapsto \R^{n \times n}$ that satisfies
%\[J\br{x,u}z=\br{\left.\frac{\partial f}{\partial x}\right|_{x,u}}z=2Q\qud{x}{z}{u}+L\br{u}z \quad \forall x,z\in\R^n,u\in \R^k\]
%Note that $J: \R^n \times \R^k \mapsto \R^{n \times n}$ is bilinear in $x$ and $u$.
%\end{definition}
\begin{figure}[htb]
\centering \includegraphics[width=.8\columnwidth]{ConvexInner.png}
\caption{Convex inner approximation of true feasible set}\label{fig:ConvexInner}
\end{figure}
We are given a nominal solution $\br{x^\star,u^\star}$ to \eqref{eq:Quad} and are interested in characterizing a convex region in $\R^k$ containing $u^\star$ such that the system is guaranteed to have a solution with
$x \in \Xcal$ (see figure \ref{fig:ConvexInner}).

\begin{assumption}
Given any norm $\norm{\cdot}$ and $x^\star \in \mathrm{Int}(\Xcal)$, it is easy to compute $r$ such that $\{x:\norm{x-x^\star}\leq r\}\subseteq \Xcal$
\end{assumption}
Given this assumption, we will henceforth assume that $\Xcal$ is always replaced by a norm ball ($\norm{x-x^\star}\leq r$) (since if we guarantee the existence of a solution within the norm ball, we guarantee a solution within $\Xcal$). While this may introduce some conservatism, most natural convex constraints can be rewritten as norms (box constraints, ellipsoidal constraints etc.).

Our main tool for computing inner approximations of $\Ucal$ is Brouwer's fixed-point theorem, which guarantees provides a sufficient condition for the existence of solutions to nonlinear systems within symmetric convex sets.
\begin{theorem}[Brouwer's fixed-point theorem]
Let $F: \R^n \mapsto \R^n$ be a continuous mapping and $S \subset \R^n$ be a compact convex set. Then, if
\begin{align*}
F\br{y} \in S \quad \forall y \in S
\end{align*}
then $F\br{y}=y$ has a solution in $S$.
\end{theorem}
Note that this is a generalization the intermediate value theorem which applies to the $n=1$ case.



==> MainResults.tex <==
\section{Inner approximations of the solvability region}\label{sec:MainResults}

In this section, we state our main theoretical results characterizing inner approximations of $\Ucal$. We then discuss tightness of these inner approximations (how far they are from the true boundary of $\Ucal$) and how they generalize previous results in the literature.

Our main result shows that given \emph{any} feasible solution of $\br{x^\star,u^\star}$ of $f\br{x,u}=0$, we can construct a family of convex regions containing $u^\star$ and a finite volume around it for which existence of a solution within distance $r$ from $x^\star$ is guaranteed. The formal result follows:
\begin{theorem}\label{thm:MainCert}
Let $\br{x^\star,u^\star}$ satisfy \eqref{eq:Quad}. Define the following quantities:
\begin{align*}
&J\br{y,u}  = 2Q(y,x^\star,u)+L\br{y,u},J\br{y,u^\star}=J^\star y\\
& \inv{J^\star}=M^\star\\
& e\br{u-u^\star}  =\norm{M^\star\br{f\br{x^\star,u}-f\br{x^\star,u^\star}}} \\
& h\br{u} =\max_{\norm{z}\leq 1} \norm{M^\star Q\qud{z}{z}{u}} \\
& g\br{u-u^\star}=\max_{\norm{z}\leq 1} \norm{\inv{J^*}\br{J\br{z,u}-J\br{z,u^\star}}}
\end{align*}
Suppose $J^*$ is nonsingular. Define the sets:
\begin{subequations}\label{eq:Cert}
\begin{align}
&\Ucal^i(\delta)=\left\{u: r\delta h\br{u}+ g\br{u-u^\star}+\frac{1}{r\delta}e\br{u-u^\star}	\leq 1 \right\} \label{eq:CertConvex}\\
&\Ucal^i = \displaystyle\cup_{0< \delta \leq 1} \Ucal^i(\delta)
\end{align}
\end{subequations}
Then for each $u \in \Ucal^i$, there is a solution to \eqref{eq:Quad} with $\norm{x-x^\star}\leq r$. Further, $\Ucal^i(\delta)$ is a convex set and hence $\Ucal^i$ is a union of convex sets. Finally, $u^\star \in \Ucal^i$ and $\Ucal^i$ is a non-empty set with positive volume.
\end{theorem}
\begin{proof}
See appendix section \ref{sec:ProofMainCert}.
\end{proof}


We now interpret the terms that appear in condition \eqref{eq:CertConvex}:
\begin{itemize}
  \item[1] $h(u)$ is a measure of how ``nonlinear'' the system is, since it bounds the \emph{gain of the quadratic term}, or the maximum norm of $Q\br{dx,dx,u}$ given inputs $dx$ within the unit ball $\norm{dx}\leq 1$. Thus, the more nonlinear the system is, the more difficult it is to satisfy \eqref{eq:CertConvex}.
  \item[2] $J\br{y,u}$ is equal to $\frac{\partial f}{\partial x} y$ and hence represents the Jacobian of the system of nonlinear equations. $J^\star$ represents the Jacobian of the system evaluated at the nominal solution $\br{x^\star,u^\star}$. Rescaling by the inverse of $J^\star$ ensure that our conditions are affine-invariant (invariant to an affine scaling of the equations). The term $g\br{u-u^\star}$ bounds the change in the Jacobian at $x^\star$ as we move from $u$ to $u^\star$ - this quantifies how a linear approximation of the equations at $x^\star$ (given by the Jacobian) changes with $u$. The condition requires this change to be small as well.
  \item Finally, the term $e\br{u-u^\star}$ quantifies how far $x^\star$ is from being a solution to $f\br{x,u}=0$, since $e\br{u-u^\star}=\norm{M^\star\br{f\br{x^\star,u}-f\br{x^\star,u^\star}}}$. The conditions requires that $x^\star$ is ``sufficiently close'' to being a solution to $f\br{x,u}=0$, or equivalently, that $u^\star$ is ``sufficiently close'' to $u$.
\end{itemize} 
\subsection{Tightness of the certificate}
We now provide a partial converse to this theorem for the special case when the quadratic and linear terms do not depend on $u$. Thus, we assume $Q\qud{x}{x}{u}=Q\br{x,x},L\br{u,x}=Lx$ for all values of $u$. Thus \eqref{eq:Quad} simplifies to
\begin{align}
Q\br{x,x}+Lx+c\br{u}=0\label{eq:QuadSimple}
\end{align}
\begin{theorem}\label{thm:Converse}
Let $\br{x^\star,u^\star}$ satisfy \eqref{eq:QuadSimple}. Define
\[e\br{u-u^\star},J^*,h\br{u}=h^\star=\max_{\norm{dx} \leq 1} \norm{\inv{J^\star}Q\br{dx,dx}}\]
as in theorem \ref{thm:MainCert}.
For any $\delta \in (0,1)$, the system of equations \eqref{eq:QuadSimple} has a solution in the set
\[\mathcal{B}_\delta=\left\{x:\norm{x-x^\star} \leq \frac{\sqrt{\delta}}{2h^*}\right\}\]
if $u$ satisfies:
\begin{align}
e\br{u-u^\star} \leq \frac{\delta}{4h^\star}\label{eq:CertSimple}
\end{align}
Conversely, if
\begin{align}
e\br{u-u^\star} > \frac{2\sqrt{\delta}+\delta}{4h^\star}\label{eq:CertSimple}
\end{align}
then \eqref{eq:QuadSimple} does not have a solution in $\mathcal{B}_\delta$.
\end{theorem}


\subsection{Relationship to previous results}

==> Numerics.tex <==
\section{Numerical results}\label{sec:NumRes}


==> Structural.tex <==
\section{Structual Properties}
\label{Sec:Properties}

\begin{comment}
\subsection{Linking the two results together}

Let $F\br{\Vlog}$ be the vector valued function with components:


\begin{theorem}\label{thm:thmLink}
The Jacobian matrix $\frac{\partial F}{\partial \Vlog}$ is equal to the LHS of \eqref{eq:EnergyFunCondvcsa} with $\cx_i=\sqrt{\Vset_i\Vset_{\Par{i}}-{\sx_i}^2}$.
\end{theorem}
\begin{proof}
This is just a straightforward calculation that follows from taking partial derivatives $\frac{\partial F_i}{\partial \Vset_j}$ for all $\br{i,j}\in \{1,\ldots,n\}$ and substituting $\cx_i=\sqrt{\Vset_i\Vset_{\Par{i}}-{\sx_i}^2}$ in \eqref{eq:EnergyFunCondvcsa}
\end{proof}

{\tb In order to link the existence of power flow solutions, we will need some results from Matrix Analysis. The results presented here are taken from \cite{PLEMMONS1977175} and \cite[Chapter 6]{AB-RJP:94}. Recall that a matrix $A \in \R^{n \times n}$ is called a Z-matrix if $A_{ij}\leq 0$ for all $i \neq j$ ($A$ has non-positive off-diagonal elements), and $A$ is called an M-matrix if it can be written as $A=sI-B$ where $s>\sigma_{\max}\br{B},B>=0$.



The following result is from Lavaei, Rantzer \& Low. It says that not-necessarily convex quadratic programs can be solved exactly by an SDP relaxation if the matrices in the quadratic program are Metzler.

\begin{lemma}
Let $M_0,\ldots, M_k$ be Metzler matrices and let $b_1,\ldots,b_k \in \mathbb{R}$. Then the following two problems have the same optimal value:
\begin{subequations}\label{Eq:MetzlerOpt1}
\begin{align}
\maxi_{x} & \quad x^{\sf T}M_0x \\
\text{Subject to }& x \in \mathbb{R}^n_{\geq 0}\\
& x^{\sf T}M_k x \geq b_k\,,\qquad k \in \{1,\ldots,K\}
\end{align}
\end{subequations}
and
\begin{subequations}\label{Eq:MetzlerOpt2}
\begin{align}
\maxi_{\Vset} & \quad \mathrm{Tr}(M_0X) \\
\text{Subject to }& X \succeq 0\\
& \mathrm{Tr}(M_kX) \geq b_k\,, \qquad k \in \{1,\ldots,K\}
\end{align}
\end{subequations}
\end{lemma}


Note to DJ: The following lemma characterizes singular M-matrices, which may be useful for arguing about what happens when the LMI is only marginally satisfied.

\begin{lemma}[\cite{AB-RJP:94}]\label{lem:Z2}
Let $A \in \mathbb{R}^{n \times n}$ be a singular irreducible M-matrix. Then
\begin{itemize}
\item[1] $A$ has rank $n-1$;
\item[2] There exists $x >\!\!> 0$ such that $Ax = 0$;
\item[3] Each principal submatrix of $A$ other than $A$ itself is a nonsingular $M$-matrix
\item[4] $A$ is \emph{almost monotone}, meaning that $Ax \geq 0 \quad \Longrightarrow \quad Ax = 0$.
\end{itemize}
\end{lemma}
}	

\begin{theorem}
If the optimization problem \eqref{eq:Opt} is feasible, its optimal solution must satisfy \eqref{eq:EnergyFunCondvcs}. Thus, if there is a solution to the power flow equations, there must be one inside the domain of convexity of the energy function. Conversely, if there are no solutions to the power flow equations inside the domain of convexity of the energy function, there are no solutions to the power flow equations anywhere. Further, if the solution exists and is in the interior of the domain of convexity of the energy function, it a unique high-voltage solution - all other solutions of the PF equations have voltage magnitudes lower than this solution at every bus.
\end{theorem}
\begin{proof}
We can rewrite \eqref{eq:Opt} equivalently as
\begin{align*}
\mini & \quad - \tran{\One}\Vlog \\
\text{Subject to } & \quad \frac{1}{2}F\br{\Vlog} \leq q
\end{align*}
since there is a monotonic relationship between $\Vlog$ and $\Vset$:$\Vset=2\expb{\Vlog}$. Further, the above optimization problem is also a convex optimization problem. Hence, the optimal solution $\Vlog^\star$ must satisfy the KKT conditions. Hence, $\exists \lambda \geq 0$ such that
\[\tranb{\left. \frac{\partial F}{\partial \Vlog}\right|_{\Vlog=\Vlog^\star}}\lambda = \One\]
It is easy to see that $\left. \frac{\partial F}{\partial \Vlog}\right|_{\Vlog=\Vlog^\star}$ is a Z-matrix. By the above condition and theorem \ref{thm:Z}, the Z-matrix must be an M-matrix and hence positive definite. Thus, by theorem \ref{thm:thmLink}, the solution is within the domain of convexity of the energy function.

Since theorem \eqref{thm:Conv} establishes the equivalence between existence of a solution and feasibility of \eqref{eq:Opt}, existence of a solution is equivalent to existence within the domain of convexity of the energy function.

Finally, if a solution $\Vset^\star$ exists in the interior of the domain of convexity of the energy function, it must be the optimal solution to \eqref{eq:Opt} (since it satisfies the KKT conditions). However, it is also the optimal solution to a whole family of problems where the uniform weight vector $\One$ is replaced with an aribtrary weight vector $w>0$. Hence, for any feasible solutions $\Vset$ of \eqref{eq:Opt} (which includes all power flow solutions), the solution $\tran{w}\br{\Vset^\star-\Vset}\geq 0$ for all $w\geq 0$. Hence, $\Vset^\star\geq \Vset$ for every other power flow solution $\Vlog$.
\end{proof}
\end{comment}
